Co-lexicographically Ordering Automata and Regular Languages -- Part II

In the present work, we tackle the regular language indexing problem by first studying the hierarchy of $p$-sortable languages: regular languages accepted by automata of width $p$. We show that the hierarchy is strict and does not collapse, and provide (exponential in $p$) upper and lower bounds relating the minimum widths of equivalent NFAs and DFAs. Our bounds indicate the importance of being able to index NFAs, as they enable indexing regular languages with much faster and smaller indexes. Our second contribution solves precisely this problem, optimally: we devise a polynomial-time algorithm that indexes any NFA with the optimal value $p$ for its width, without explicitly computing $p$ (NP-hard to find). In particular, this implies that we can index in polynomial time the well-studied case $p=1$ (Wheeler NFAs). More in general, in polynomial time we can build an index breaking the worst-case conditional lower bound of $\Omega(|P| m)$, whenever the input NFA's width is $p \in o(\sqrt{m})$.

==> path_orders.tex <==
\subsection{Path orders}

We start by relaxing the notion of co-lexicographic order. Intuitively, we deem states reached by the same strings ($u,v$ with $I_u=I_v$) always comparable, regardless of whether or not they satisfy the co-lexicographic axioms.

\begin{comment}

Let $ \mathcal{A} = (Q, \delta, s, F) $ be an NFA. For every $ u \in Q $, let $ \lambda(u) \subseteq \Sigma $ be the set of all characters labeling some edge reaching $ u $ \notaN{mettere in sez 2.1}. For $ u, v \in Q $, define:
\begin{equation*}
    \lambda(u) \preceq \lambda (v) \iff (\forall a \in \lambda(u))(\forall b \in \lambda (v))(a \preceq b)
\end{equation*}

\notaN{sopra c'è la def di NicolaC, ma credo debba essere come sotto:}

\begin{equation*}
    \lambda(u) \preceq \lambda (v) \iff (\forall a \in \lambda(u))(\forall b \in \lambda (v))(\{a,b\} \not\subseteq \lambda(u) \cap \lambda(v) \rightarrow a\prec b)
\end{equation*}

\notaN{Nota: ho dato la definizione \ref{def:path order} in versione locale, perchè in realtà la globale (Lem \ref{lem:path order global}) mi pare valga solo per la relazione reduced.}

\begin{definition}\label{def:path order}
Let $ \mathcal{A} = (Q, \delta, s, F) $ be an NFA, $ \le $ be a partial order on $ Q $, and $\equiv$ be an equivalence relation over $Q$ such that $u \equiv v \Rightarrow I_u = I_v$. Fix moreover an arbitrary bijective function (an enumeration) $\pi: Q\rightarrow [1,|Q|]$.
We say that $ \le $ is a $(\equiv,\pi)$-path-order on $ \mathcal{A} $ if for every $ u, v \in Q $ the following properties hold:

\begin{enumerate}
    \item If $u<v$, then $ v \neq s $;
    \item If $u<v$, then $ \lambda(u) \preceq \lambda (v) $;
    \item If $u\equiv v$, then $u<v$ if and only if $\pi(u) < \pi(v)$;
    \item If $u<v$ and $u\not\equiv v$, then for every $ u', v' \in Q $ such that $u'\not\equiv v'$ and for every $ a \in \Sigma $, the following holds: if $ u \in \delta(u', a) $ and $ v \in \delta(v', a) $, then $ u' < v' $.
\end{enumerate}
\end{definition}

Path orders have the following more intuitive "global" interpretation, which will turn out to be useful in the following proofs. 

\end{comment}


Importantly, note that the following definition does not impose any constraint on the order of pairs $u,v$ such that $u\not\equiv v$ and $u \equiv_{\mathcal A} v$. 

\notaN{nota: $\equiv_{\mathcal A}$ è la relazione reduced}

\begin{definition}\label{lem:path order global}
Let $ \mathcal{A} = (Q, \delta, s, F) $ be an NFA, $ \le $ be a partial order on $ Q $, and $\equiv$ be an equivalence relation over $Q$ such that $u \equiv v \Rightarrow I_u = I_v$. Fix moreover an arbitrary bijective function (an enumeration) $\pi: Q\rightarrow [1,|Q|]$.
We say that $<$ is a $(\equiv,\pi)$-path-order if and only if it satisfies the following two properties:
\begin{enumerate}
    \item If $u\equiv v$, then $u<v$ if and only if $\pi(u) < \pi(v)$;
    \item If $u\not\equiv_{\mathcal A} v$, then $u<v$ if and only if $(\forall \alpha\in I_u,\ \forall\beta\in I_v\ :\ \{\alpha,\beta\} \not\subseteq I_u \cap I_v \rightarrow \alpha \prec \beta)$.
\end{enumerate}
\end{definition}





The following property is a weaker version of the \emph{path coherency} property possessed by co-lexicographic orders \cite{cotumaccio2021indexing}. 
While path coherency states that following equally-labeled edges from \emph{any} interval in $(Q,<)$ leads to another interval in $(Q,<)$, in the following lemma we restrict our attention to intervals reached by strings suffixed by a given fixed string $P$. 
As we show next, this weaker form of path coherency is actually still sufficient for indexing. 



\notaN{TODO notazione $P \supseteq \alpha$ per indicare che P è suffisso di $\alpha$}.





\begin{lemma}
Let $\le$ be a path order for the NFA $\mathcal A = (Q,s,\Sigma,\delta,F)$. Let moreover $U(P)$ be the set formed by all the states reached by a path suffixed by a given string $P$:  $U(P) = \{q\ :\ \exists \alpha\in I_q,\ P \supseteq \alpha\}$. Then, $U(P)$ is an interval in $(Q,\le)$.
\end{lemma}
\begin{proof}
We prove the property by induction on the length $m = |P|$ of $P$. If $m=0$, $P$ is the empty string and the property clearly holds: $U(P) = Q$ (all states are reached by a path suffixed by the empty string), and $Q$ is the full interval on $(Q,\le)$.

Assume inductively that the property holds for $P$ of length $m$. Let $P'=P\cdot a$, for any $a\in \Sigma$, and consider the set $U(P')$ of all states reached by a path suffixed by $P'$. Our goal is to prove that $U(P')$ is an interval on $(Q,\le)$.

Assume, for contradiction, that $U(P')$ is not an interval on $(Q,\le)$.
Then, there exist three comparable (distinct) states $u < v < w$ such that $u,w \in U(P')$ and $v \notin U(P')$. 
%Note that $v$ cannot be the initial state $s$ by condition (1) of Definition \ref{def:path order}. 
Let $\equiv_{\mathcal A} \subseteq Q\times Q$ be the relation defined as $u \equiv_{\mathcal A} v$ if and only if $I_u = I_v$. \notaN{TODO mettere questa definizione (relazione reduced) in sez. 2.1}. 

\begin{claim}\label{claim:uvw}
$u \not \equiv_{\mathcal A} v \not \equiv_{\mathcal A} w$.
\end{claim}
\begin{proof}
If it were $u \equiv_{\mathcal A} v$ or $v \equiv_{\mathcal A} w$, then by definition of $\equiv_{\mathcal A}$, it would be $I_u = I_v$ or $I_v = I_w$. In both cases, $v$ would be reached by at least one string suffixed by $P'$ (and hence $v \in U(P')$), since both $u$ and $w$ are reached by at least one string suffixed by $P'$. 
\end{proof}
 


\begin{claim}
$u \not\equiv_{\mathcal A} w$
\end{claim}
\begin{proof}
Assume, for contradiction, that $u \equiv_{\mathcal A} w$. 
%Note that this implies that $u \neq s$.
We distinguish two cases. 

(a) $I_v \subset I_u = I_w$. Let $\alpha \in I_u \setminus I_v$, and pick any $\beta \in I_v$. Note that 
$\{\alpha, \beta\} \not\subseteq I_u \cap I_v$.
Since $u \not\equiv_{\mathcal A} v$ (Claim \ref{claim:uvw}), then by Property (2) of Lemma \ref{lem:path order global} it must be the case that $\alpha \prec \beta$ (otherwise it would be $v<u$).
However, from $u \equiv_{\mathcal A} w$ we deduce that $\alpha \in I_w$ as well, and  $\{\alpha, \beta\} \not\subseteq I_v \cap I_w$. Then, since $\alpha \prec \beta$ and $v \not\equiv_{\mathcal A} w$ (Claim \ref{claim:uvw}), by Property (2) of Lemma \ref{lem:path order global} we deduce $w < v$, a contradiction.

(b) $I_v \not\subset I_u = I_w$. Then, there must be a string $\beta \in I_u \setminus I_v$. Pick any $\alpha \in I_v = I_w$. Since $\{\alpha, \beta\} \not\subseteq I_u \cap I_v$ and $\{\alpha, \beta\} \not\subseteq I_v \cap I_w$, the same reasoning of case (a) can be applied to obtain a contradiction. 
\end{proof}

Recall that $P' = P\cdot a$. We furthermore show:

\begin{claim}
$a \in \lambda(v)$.
\end{claim}
\begin{proof}
Assume, for contradiction, that $a \notin \lambda(v)$. Note that $a \in \lambda(u) \cap \lambda(w)$ (because $P\cdot a \in I_u \cap I_w$). Take any $\gamma \in \lambda(v)$. By assumption, $\gamma \neq a$. If $\gamma \prec a$, then take any $\alpha\cdot a\in I_u$ and $\beta\cdot \gamma \in I_v$. Since $a\notin\lambda(v)$, we have $\{\alpha\cdot a, \beta\cdot \gamma\} \notin I_u\cap I_v$. Moreover, since $\gamma \prec a$ then $\beta\cdot \gamma \prec \alpha\cdot a$. Finally, $u \not\equiv_{\mathcal A} v$ and property (2) of Lemma \ref{lem:path order global} imply $u\not < v$, a contradiction. On the other hand, if $a \prec \gamma$ then by a similar reasoning we obtain $v\not<w$, again a contradiction. This proves our claim.
\end{proof}


Take now $\alpha\cdot a \in I_u$ such that $P\cdot a \supseteq \alpha\cdot a$. Consider any $\beta\cdot a \in I_v$. By assumption,  $P\cdot a \not\supseteq \beta\cdot a$ (because $v \notin U(P\cdot a)$). Then, $\{\alpha\cdot a, \beta\cdot a\} \not\subseteq I_u\cap I_v$. By Property (2) of Lemma \ref{lem:path order global}, we  deduce $\alpha\cdot a \prec \beta\cdot a$ (and thus $\alpha \prec \beta$).
Denote $u', v'$ two $a$-predecessors of $u,v$, respectively, such that $\alpha \in I_{u'}$  and $\beta \in I_{v'}$. Note that $P \supseteq \alpha$. At the same time, it cannot be $P \supseteq \beta$ as this would imply $P\cdot a \supseteq \beta\cdot a$ and thus $v \in U(P\cdot a) = U(P')$. This implies that $\{\alpha,\beta\} \not \subseteq I_{u'} \cap I_{v'}$ and then, by 
Property (2) of Lemma \ref{lem:path order global} we deduce $u'<v'$. Repeating the same reasoning for $w$, we deduce that there exists an $a$-predecessor $w'$ of $w$ such that  $u'<v'<w'$ and there exists a string $\alpha' \in I_{w'}$ suffixed by $P$ (that is, $P \supseteq \alpha'$). We apply the inductive hypothesis on $P$, of length $m$, and obtain that $U(P)$ is a $(Q,\le)$-interval. This means that $P \supseteq \beta'$, for some $\beta' \in I_{v'}$. But then, this implies that $\beta'\cdot a \in I_v$, with $P' = P\cdot a \supseteq \beta'\cdot a$, i.e. $v\in U(P\cdot a) = U(P')$: a contradiction. Since the original (absurd) hypothesis was that $U(P')$ is not an interval in $(Q,\le)$, this proves the claim for pattern length $m+1 = |P'|$, completing the inductive proof.
\end{proof}

